Safety-Critical Coordination for Cooperative Legged Locomotion via Control Barrier Functions

This paper presents a safety-critical approach to the coordinated control of cooperative robots locomoting in the presence of fixed (holonomic) constraints. To this end, we leverage control barrier functions (CBFs) to ensure the safe cooperation of the robots while maintaining a desired formation and avoiding obstacles. The top-level planner generates a set of feasible trajectories, accounting for both kinematic constraints between the robots and physical constraints of the environment. This planner leverages CBFs to ensure safety-critical coordination control, i.e., guarantee safety of the collaborative robots during locomotion. The middle-level trajectory planner incorporates interconnected single rigid body (SRB) dynamics to generate optimal ground reaction forces (GRFs) to track the safety-ensured trajectories from the top-level planner while addressing the interconnection dynamics between agents. Distributed low-level controllers generate whole-body motion to follow the prescribed optimal GRFs while ensuring the friction cone condition at each end of the stance legs. The effectiveness of the approach is demonstrated through numerical simulations and experimentally on a pair of quadrupedal robots.

==> util_jeeseop.tex <==
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{mathrsfs}
\usepackage{graphicx} % for pdf, bitmapped graphics files
%\usepackage[draft]{graphicx} % for pdf, bitmapped graphics files
%\usepackage[caption=false,labelformat=parens]{subfig}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{svg}
\usepackage{xcolor}
\usepackage{bm}
\usepackage{cite}

% Define commands
\newtheorem{theorem}{\textbf{Theorem}}
\newtheorem{lemma}{\textbf{Lemma}}
\newtheorem{corollary}{\textbf{Corollary}}
\newtheorem{assumption}{\textbf{Assumption}}
\newtheorem{definition}{\textbf{Definition}}
\newtheorem{example}{\textbf{Example}}
\newtheorem{remark}{\textbf{Remark}}
\newtheorem{problem}{Problem}

% Special commands
\newcommand{\Real}{\mathbb R}
\newcommand{\Tau}{\mathrm{T}}
\newcommand{\Integer}{\mathbb{Z}_{\geq0}}
\newcommand{\col}{\textrm{col}}
\newcommand{\ol}{\textrm{ol}}
\newcommand{\cl}{\textrm{cl}}
\newcommand{\inte}{\textrm{int}}
\newcommand{\Lie}{\textrm{L}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\eq}{\textrm{eq}}
\newcommand{\ineq}{\textrm{ineq}}
\newcommand{\iden}{\mathbb{I}}
\newcommand{\net}{\textrm{net}}
\newcommand{\vect}{\textrm{vec}}
\newcommand{\op}{\textrm{op}}
\newcommand{\des}{\textrm{des}}
\newcommand{\dyn}{\textrm{dyn}}
\newcommand{\hol}{\textrm{hol}}
\newcommand{\con}{\textrm{con}}
\newcommand{\inter}{\textrm{int}}

\newcommand{\gap}{\vspace{0.1cm}}
\DeclareMathOperator*{\argmin}{argmin}
